TAMP: Token-Adaptive Layerwise Pruning in Multimodal Large Language Models

Multimodal Large Language Models (MLLMs) have shown remarkable versatility in understanding diverse multimodal data and tasks. However, these capabilities come with an increased model scale. While post-training pruning reduces model size in unimodal models, its application to MLLMs often yields limited success. Our analysis discovers that conventional methods fail to account for the unique token attributes across layers and modalities inherent to MLLMs. Inspired by this observation, we propose TAMP, a simple yet effective pruning framework tailored for MLLMs, featuring two key components: (1) Diversity-Aware Sparsity, which adjusts sparsity ratio per layer based on diversities among multimodal output tokens, preserving more parameters in high-diversity layers; and (2) Adaptive Multimodal Input Activation, which identifies representative multimodal input tokens using attention scores to guide unstructured weight pruning. We validate our method on two state-of-the-art MLLMs: LLaVA-NeXT, designed for vision-language tasks, and VideoLLaMA2, capable of processing audio, visual, and language modalities. Empirical experiments across various multimodal evaluation benchmarks demonstrate that each component of our approach substantially outperforms existing pruning techniques.

==> materials/figures/3_attention_trend.tex <==
\begin{figure}[t]
    \centering
    \small
    \includegraphics[width=0.9\linewidth]{figures/attention_trend/attention_trend_refine.pdf}
    \par
    \vspace{-0.05in}
    \caption{\small Average attention score across LLaVA-NexT blocks. Varying attention score indicates that the model there exist unique processing demands of each block.}
    \label{fig:attention_trend}
    \vspace{-0.1in}
\end{figure}

==> materials/tables/3_token_selection_ablation.tex <==
\begin{table}[t]
    \tiny
    \caption{\small Impact of token selection on 50\% pruning of LLaVA-NeXT across evaluation benchmarks. MME measures general multimodal understanding, while ChartQA focuses on visually rich information understanding (e.g., OCR, chart).}
    \vspace{-0.075in}
    \centering
    \resizebox{\linewidth}{!}{
        \renewcommand{\arraystretch}{1.1}
        \renewcommand{\tabcolsep}{2pt}
        \begin{tabular}{l c c c c}
             \toprule
             {\textbf{Method}} & {\textbf{MME-}} & {\textbf{MME-}} & {\textbf{ChartQA}} \\
             & {\textbf{Cognition}} & {\textbf{Perception}} & \\
             \midrule
             Full Model &
             {\scriptsize 376.8} & {\scriptsize 1588.3} & {\scriptsize 69.2}\\
              \cmidrule{0-4}
             All tokens (Block 1 - 32) &
             {\scriptsize 276.4} & {\scriptsize 1360.6} & {\scriptsize 63.2}\\
             V+L (Block 1 - 32) &
             {\scriptsize 249.6} & {\scriptsize 1419.8} & {\scriptsize \textbf{63.4}}\\
             V+L (Block 1 - 2), L (Block 3 - 32) &
             {\scriptsize \textbf{337.5}} & {\scriptsize \textbf{1476.2}} & {\scriptsize 62.4}\\
             L (Block 1 - 32) &
             {\scriptsize 302.9} & {\scriptsize 1427.4} & {\scriptsize 62.8}\\
             \bottomrule
        \end{tabular}
    }
    \label{tab:token_selection_ablation}
    \vspace{-0.1in}
\end{table}
